A Survey on In-context Learning

With the increasing capabilities of large language models (LLMs), in-context learning (ICL) has emerged as a new paradigm for natural language processing (NLP), where LLMs make predictions based on contexts augmented with a few examples. It has been a significant trend to explore ICL to evaluate and extrapolate the ability of LLMs. In this paper, we aim to survey and summarize the progress and challenges of ICL. We first present a formal definition of ICL and clarify its correlation to related studies. Then, we organize and discuss advanced techniques, including training strategies, prompt designing strategies, and related analysis. Additionally, we explore various ICL application scenarios, such as data engineering and knowledge updating. Finally, we address the challenges of ICL and suggest potential directions for further research. We hope that our work can encourage more research on uncovering how ICL works and improving ICL.

==> fig/table_sketch.tex <==
\begin{table}[t]                
\centering      
\setlength{\tabcolsep}{2pt}  
{  \fontsize{9pt}{11pt}\selectfont          
\begin{tabular}{lccccccc}      
\toprule             
\bf Model & \bf Method & \bf SST5 &  \bf SST2 & \bf CQA  & \bf SNLI & \bf News & \bf Avg \\       
\midrule             
\multirow{3}{*}{GPT2}          
% & random & 25.6 & 53.5 & 34.2 & &25.4 & \\            
& topk & 40.1 & 74.9 & 30.2 & 39.7&62.7 & 49.5\\            
& votek & 32.4 & 51.0 & 29.8 & 35.8& 25.5 & 34.9 \\            
& mdl & \textbf{43.3} & \textbf{86.7} & \textbf{32.7} & \textbf{41.4}& 
\textbf{68.0} & \textbf{54.4}\\       
\midrule             
\multirow{3}{*}{GPT-J}              
% & random & 37.6 & 84.0 & 64.1 & &35.9 & \\            
& topk & \textbf{46.9} & 84.6 & 58.4 & \textbf{60.7} & \textbf{69.1} & \textbf{63.9} \\            
& votek & 33.8 & 87.3 & 63.4 & 43.1& 25.3 & 50.6\\            
& mdl & 37.6 & \textbf{87.9} & \textbf{64.1} & 59.8  & 68.2 &63.5\\        
\midrule              
\multirow{3}{*}{Qwen2}        
% & random & 52.9 & 80.1 & 76.9 & &56.3 & \\            
& topk & 54.1 & 83.3 & 76.3 & \textbf{68.2} &64.9 &  \textbf{69.4}\\            
& votek & \textbf{55.3} & \textbf{86.9} & 76.1 &51.6& \bf 65.3 & 67.0\\            
& mdl & 54.6 & 86.1 & \textbf{77.1} &65.0& 63.2 &69.2\\            
\midrule             
\multirow{3}{*}{Llama3}              
% & random & 51.5 & 88.3 & 74.3 & & 75.2  & \\      
& topk & 53.0 & \textbf{90.3} & 76.1 & \textbf{64.0} & 74.0 &  \textbf{71.5}\\            
& votek & 54.9 & 88.9 & 72.6 & 57.7& \textbf{78.3} & 70.5\\            
& mdl & \textbf{54.4} & 89.1 & \textbf{76.5} & 59.9 & 74.6 &70.9 \\               
\bottomrule                
\end{tabular}}                   
\caption{Fair comparison of demonstration selection methods. CQA and News are abbreviations of Commonsense QA and AG News, respectively. The best results are \textbf{bolded}. Our experiments on topk~\citep{liu2022close}, votek~\citep{su2022selective}, mdl~\citep{Wu2022SelfadaptiveIL} 
show that the effectiveness of ICL example selection methods are model-dependent. On GPT-2, the mdl method performs the best, while on the other three models,
topk performs the best.
%show that topk selects the most effective examples on average.
}    
\label{tab:experiment_design_centered_model_names}        
\end{table} 

==> sections/020overview.tex <==
% \qingxiu{Modifying...}
%As illustrated in Figure~\ref{taxo_of_icl}, 
The strong performance of ICL relies on two stages: (1) the training stage that cultivates the ICL ability of LLMs, and (2) the inference stage where LLMs predict according to task-specific demonstrations.
%In terms of the training stage, pretraining is significant for bringing up the ICL ability and the optional warmup can further improve the ICL ability.
%In terms of the training stage, the language models are pretrained with 
In terms of the training stage, LLMs are directly trained on language modeling objectives, such as left-to-right generation. Although the models are not specifically optimized for in-context learning, they still exhibit the ICL ability.
% \leiModify{the logic here seems not very clear?} 
Existing studies on ICL basically take a well-trained LLM as the backbone, and thus this survey will not cover the details of pretraining language models. 
Towards the inference stage, as the input and output labels are all represented in interpretable natural language templates, there are multiple directions for improving ICL performance. 
% This paper will give a detailed description and comparison, such as selecting suitable examples for demonstrations and designing specific scoring methods for different tasks.
%Given a pretrained LLM and a well-designed demonstration, various scoring methods can be adopted for particular tasks.
% As illustrated in Fig.~\ref{fig:icl_process}, the LLM and the demonstration are two crucial components of ICL.
% In terms of the LLM, the pretraining stage is significant for bringing up the ICL ability and the optional warmup stage can further improve the ICL ability.
% Towards the demonstrations, as the input and output labels are all represented in interpretable language tokens, humans could design better promptings strategies such as selecting suitable examples for demonstrations and decomposing the reasoning procedure in text for hinting the model.
% Given a pretrained LLM and a well-designed demonstration, various scoring methods can be adopted for particular tasks.
% ICL consists of four main stages: (1) LLMs pretraining that ; (2) optional model warm-up that; (3) demonstration designing that (4) scoring. The main procedures are 
% detection to identify claims that require verification; (ii) evidence retrieval to find sources
% supporting or refuting the claim; and (iii) claim
% verification to assess the veracity of the claim
% based on the retrieved evidence. 
%With the formulation, 
% We notice that there are important components in the framework. 
% First, the core of in-context learning is the model itself, whose model scale and pretraining corpus have a great influence on the final prediction performance.
% % We discuss various model training techniques for improving the ICL ability of the model proposed in \S~\ref{sec:warmup}.
% Besides, as the input and output labels are all represented in interpretable language tokens, humans could design better promptings strategies such as selecting suitable examples for demonstrations and decomposing the reasoning procedure in text for hinting the model.
% % which we provide an overview of current progress in \S\ref{sec:prompt_designing}. 

% \leiModify{How to connect to the rest parts of this paper?}

% Structure of this paper
% With the rapid development of ICL,
We organize the current progress in ICL following the taxonomy above (as shown in Figure~\ref{taxo_of_icl}). 
With a formal definition of ICL~(\S\ref{sec:formulation}), 
% by providing a comprehensive
% birds-eye view of the area and formal definition of in-context learning methods~(\S\ref{sec:formulation}).
we provide a detailed discussion of the ICL-augmented pretraining and warmup approaches~(\S\ref{sec:training}) and the demonstration designing strategies (\S\ref{sec:prompt_tuning}). \S\ref{sec:analysis} provides in-depth discussions of current explorations on unveiling the secrets behind the ICL. 
We further provide useful evaluation and resources~(\S\ref{sec:evaluation}), potential applications~(\S\ref{sec:application}) and potential challenges~(\S\ref{sec:challege_future}) in Appendix
% .and hope this could pave the way for researchers in this field.
% In this paper, we present a curated survey on the related studies of in-context learning, to give a comprehensive
% birds-eye view of the area.

% Remove Structure 
% The paper is structured as follows:
% We discuss the related work in 
% \S\ref{sec:related}, by categorising the ICL methods into three types. 
% Furthermore, we introduce the prompting strategies of ICL in \S\ref{sec:approach}, as the the design of in-context demonstrations has a great impact on the model performance. Finally, we point out several challenges and future directions to facilitate the community in \S\ref{sec:impact}.


==> tabs/tab_evaluation.tex <==
\begin{table*}[]
\small
    \centering
    \begin{tabular}{lccccccccc}
    \toprule
     ~ & \bf SuperGLUE & \bf BoolQ & \bf CB  & \bf COPA & \bf RTE  & \bf WiC  & \bf WSC  & \bf MultiRC & \bf  ReCoRD \\
 ~& Avg. & Acc. & Acc.,F1 & Acc. & Acc. &
 Acc.  & Acc. & Acc.,F1a & Acc.,F1\\
     \midrule
     Human Baseline & 89.8  & 89.0  & 95.8/98.9  & 100.0  & 81.8/51.9  & 91.7/91.3  & 93.6  & 80.0 & 100.0   \\
     Finetuned SOTA \\
     Vanilla GPT3  &   &  &   & \\
    \makecell[l]{Chain-of-thoughts \\ ~\cite{beyond}}   &   & &   & \\
    \makecell[l]{Least-to-most\\ ~\cite{suzgun2022challenging}}   & &  &   & \\
    \bottomrule
    \end{tabular}
    \caption{Benchmarking exsiting prompting strategies on the GLUE tasks with 8 demonstration examples on each dataset.}
    \label{tab:evaluation}
\end{table*}
